OASIS: Open Agent Social Interaction Simulations with One Million Agents

There has been a growing interest in enhancing rule-based agent-based models (ABMs) for social media platforms (i.e., X, Reddit) with more realistic large language model (LLM) agents, thereby allowing for a more nuanced study of complex systems. As a result, several LLM-based ABMs have been proposed in the past year. While they hold promise, each simulator is specifically designed to study a particular scenario, making it time-consuming and resource-intensive to explore other phenomena using the same ABM. Additionally, these models simulate only a limited number of agents, whereas real-world social media platforms involve millions of users. To this end, we propose OASIS, a generalizable and scalable social media simulator. OASIS is designed based on real-world social media platforms, incorporating dynamically updated environments (i.e., dynamic social networks and post information), diverse action spaces (i.e., following, commenting), and recommendation systems (i.e., interest-based and hot-score-based). Additionally, OASIS supports large-scale user simulations, capable of modeling up to one million users. With these features, OASIS can be easily extended to different social media platforms to study large-scale group phenomena and behaviors. We replicate various social phenomena, including information spreading, group polarization, and herd effects across X and Reddit platforms. Moreover, we provide observations of social phenomena at different agent group scales. We observe that the larger agent group scale leads to more enhanced group dynamics and more diverse and helpful agents' opinions. These findings demonstrate OASIS's potential as a powerful tool for studying complex systems in digital environments.

==> Section/5_ablation_study.tex <==
\section{Ablation Study}



\subsection{recommend system ablation}
%We developed a simple recommendation system (recsys). \bowen{We formulate a simplified version of RecSys in \GENSS to clearly...} And 
To verify the impact of RecSys on message dissemination, we conducted ablation studies on the existence of the RecSys itself and the RecSys model(different models to embed tweets and profiles). For these experiments, we randomly selected 28 topics from the 198 topics collected before, ensuring that they covered different areas. Notably, we only show the RMSE of scale in Figure \ref{fig:recsys ablation loss} due to space constraints, more metrics comparison can be found in Appendix \ref{appendix:Detailed Ablation results}.

\begin{figure}[H]
    \centering
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/recsys ablation.png}
        \caption{RecSys ablation results on scale Normalized RMSE, TWHIN-BERT, and regular BERT showed much better performance.}
        \label{fig:recsys ablation loss}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.45\textwidth}
        \vspace{-2pt}
        \centering
        \includegraphics[width=\linewidth]{figures/recsys ablation example.png}
        \vspace{2pt}
        \caption{Recommendation results of TwHIN-BERT and regular BERT. TWHIN-BERT can identify the relationship between Barry Allen and The Flash (Barry Allen is the second-generation Flash), whereas regular BERT would not be able to achieve this.}
        \label{fig:recsys_ablation_example}
    \end{subfigure}
    \caption{Recsys Ablation results and recommendation results comparison}
    \label{fig:recsys_combined}
\end{figure}



% \begin{wrapfigure}{r}{0.5\textwidth}\centering\includegraphics[width=0.48\textwidth]{figures/recsys ablation.png}
% \vspace{-20pt}
%     \caption{recsys ablation}
%     \label{fig:recsys_ablation}
% \end{wrapfigure}




\textbf{w/o RecSys.} 
% In our experiments, we found that removing the RecSys for certain entertainment-related topics still resulted in good simulation outcomes. This success is due to the dense follower networks that spontaneously form within fan groups who have long-term shared interests in specific topics. However, such dense networks are often absent among the groups for other types of topics. As a result, when we remove the RecSys, the information dissemination process within these groups tends to terminate prematurely, typically manifesting as broadcast behavior from a single superuser, without further propagation. In such cases, the RecSys is essential for connecting isolated nodes within the group to sustain the simulation.
In our experiments, removing the RecSys for some entertainment topics worked well due to dense follower networks in fan groups. However, most groups lack these networks, leading to premature information spread, typically manifesting as broadcast behavior from a single superuser. Thus, the RecSys is essential for connecting isolated nodes and sustaining the simulation. \textbf{Different RecSys model.} Pre-trained on over 7 billion tweets in 100+ languages, TwHIN-BERT is more suitable for recommendation systems than general models. Here we choose paraphrase-MiniLM-L6-v2 \citep{reimers-2019-sentence-bert} and BERT-base-multilingual-cased (regular BERT) \citep{DBLP:journals/corr/abs-1810-04805} for the ablation study, we can found that TWHIN-BERT and regular BERT showed much better performance than paraphrase-MiniLM-L6-v2 in Figure \ref{fig:recsys ablation loss}. Moreover, based on recommendation results in Figure \ref{fig:recsys_ablation_example}, TWHIN-BERT could recommend a more proper post.

% \textbf{w/o fan score.} Since the social network on Twitter operates as a scale-free network, enhancing the broadcast effect of super users is necessary. The reduction in max breadth RMSE loss indicates that including this fan count weighting effectively reduces the loss, making the message propagation characteristics in the sandbox environment more closely aligned with real-world scenarios.

% \textbf{w/o like score.} 
% According to the scale RMSE loss, adding the like score has little impact on message propagation during the simulation, as the RecSys can function adequately based on the similarity between user profiles and tweets in 100 minutes (33 time steps), Additionally, since incorporating the like score somewhat mitigates the broadcasting effect of super users, we can observe that the loss on the max breadth curve is larger when the like score is included.



% \subsection{LLM ablation}
% \textbf{\textcolor{red}{zirui}}
% \begin{figure}[h]
%     \centering
%     \includegraphics[width=1\linewidth]{figures/model ablation.png}
%     \caption{model ablation}
%     \label{fig:model ablation}
% \end{figure}

\subsection{temporal feature ablation}

\begin{wrapfigure}{r}{0.6\textwidth}
    \vspace{-12pt}
    \centering
    \includegraphics[width=\linewidth]{figures/GENSS-No temporal feature-Real-all_stats.png}  
    \caption{Normalized RMSE between GENSS, GENSS w/o temporal feature simulation results and real propagation}  
    
    \label{fig:temporal feature ablation rmseloss}  
\end{wrapfigure}

We ablate our temporal feature (the hourly activity level extracted from the crawled data) in this experiment. Specifically, we rerun the experiments of reproducing real-world information propagation under all activity probabilities set to 1.0 and compare their Normalized RMSE on 28 topics. We can easily see that without the temporal features, our \GENSS can not capture the dynamics of real-world information propagation well since all agents take action so frequently.


% \begin{figure}[h]
%     \centering
%     \includegraphics[width=\textwidth]{figures/GENSS-No temporal feature-Real-all_stats.png}  
%     \caption{Normalized RMSE between GENSS, GENSS w/o temporal feature simulation results and real propagation}  
%     \label{fig:temporal feature ablation rmseloss}  
% \end{figure}



% \subsection{User Generation Ablation}
% \textbf{\textcolor{red}{yuxian\&zirui}}

